A Relaxed Primal-Dual Hybrid Gradient Method with Line Search

The primal-dual hybrid gradient method (PDHG) is useful for optimization problems that commonly appear in image reconstruction. A downside of PDHG is that there are typically three user-set parameters and performance of the algorithm is sensitive to their values. Toward a parameter-free algorithm, we combine two existing line searches. The first, by Malitsky et al., is over two of the step sizes in the PDHG iterations. We then use the connection between PDHG and the primal-dual form of Douglas-Rachford splitting to construct a line search over the relaxation parameter. We demonstrate the efficacy of the combined line search on multiple problems, including a novel inverse problem in magnetic resonance image reconstruction. The method presented in this manuscript is the first parameter-free variant of PDHG (across all numerical experiments, there were no changes to line search hyperparameters).

==> app1.tex <==
\newpage

\section{Primal Dual DR with Relaxation}\label{ap:1}
\todo{I don't see where this appendix is referenced in the manuscript.  Please make sure that it is referenced.  Also, appendices should be listed in the order that they are referenced in the manuscript.}
Starting from the iterations of Douglas-Rachford but with a relaxation parameter this time:
\begin{equation*}
\begin{aligned}
    x_{k+1} &= \prox_{\gamma f}(y_k)\\
    y_{k+1}&=y_k + \rho_k\left(\prox_{\gamma g}(2x_{k+1} - y_k) - x_{k+1}\right)
\end{aligned}
\end{equation*}
Applying the Moreau decomposition to the second iteration yields the primal-dual DR:
\begin{equation*}
    \begin{aligned}
        y_{k+1} &= y_k + \rho_k\left(\prox_{\gamma g}(2x_{k+1} - y_k) - x_{k+1}\right) \\
        &= y_k + \rho_k\left(x_{k+1} - y_k - \gamma\prox_{\gamma ^{-1}g^*}\left(\frac{1}{\gamma}(2x_{k+1} - y_k)\right)\right) \\
        &= (1 - \rho_k)y_k + \rho_kx_{k+1} - \rho_k\left(\gamma\prox_{\gamma ^{-1}g^*}\left(\frac{1}{\gamma}R_{\gamma f}y_k\right)\right)\\
        &= (1 - \rho_k)y_k + \rho_kx_{k+1} \\
        &\hspace{2em} - \rho_k\gamma \left[2\prox_{\gamma ^{-1}g^*}\left(\frac{1}{\gamma}R_{\gamma f}y_k\right) - \frac{1}{\gamma}R_{\gamma f}y_k - \prox_{\gamma ^{-1}g^*}\left(\frac{1}{\gamma}R_{\gamma f}y_k\right) + \frac{1}{\gamma}R_{\gamma f}y_k\right]\\
        &= (1 - \rho_k)y_k + \rho_kx_{k+1} - \rho_k\gamma \left(R_{\gamma^{-1}g^*}\left[\frac{1}{\gamma}R_{\gamma f}y_k\right] - \prox_{\gamma ^{-1}g^*}\left(\frac{1}{\gamma}R_{\gamma f}y_k\right) + \frac{1}{\gamma}R_{\gamma f}y_k\right)\\
        &= (1 - \rho_k)y_k + \rho_kx_{k+1} - \rho_k\gamma R_{\gamma^{-1}g^*}\left[\frac{1}{\gamma}R_{\gamma f}y_k\right] - \rho_k\left(R_{\gamma f}y_k - \gamma\prox_{\gamma ^{-1}g^*}\left(R_{\gamma f}y_k\right)\right)\\
        &= (1 - \rho_k)y_k - \rho_k\gamma R_{\gamma^{-1}g^*}\left[\frac{1}{\gamma}R_{\gamma f}y_k\right] - \underbrace{\rho_k\left(x_{k+1} - y_k - \gamma\prox_{\gamma^{-1}g^*}\left(R_{\gamma f}y_k\right)\right)}_{y_{k+1} - y_k}\\
        &= (1 - \rho_k)y_k - \rho_k\gamma R_{\gamma^{-1}g^*}\left[\frac{1}{\gamma}R_{\gamma f}y_k\right] + y_k - y_{k+1} \\
        2 y_{k+1} &= (2 - \rho_k)y_k - \rho_k\gamma R_{\gamma^{-1}g^*}\left[\frac{1}{\gamma}R_{\gamma f}y_k\right] \\
        y_{k+1} &= (1 - \frac{\rho_k}{2})y_k - \frac{\rho_k}{2}\gamma R_{\gamma^{-1}g^*}\left[\frac{1}{\gamma}R_{\gamma f}y_k\right]
    \end{aligned}
\end{equation*}
This is now an averaged operator iteration with $S = -\gamma R_{\gamma^{-1}g^{*}}(\frac{1}{\gamma}R_{\gamma f})$ and $\alpha = \frac{\rho_k}{2}$. The composition of nonexpansive operators is nonexpansive, so $S$ is nonexpansive and the averaged operator iteration converges.

==> app2_ls.tex <==
\section*{Definitions}
Let $\mathcal{H}$ be a Hilbert space with inner product $\langle \, \cdot \, , \, \cdot \rangle$ and induced norm $\lVert \, \cdot \, \rVert = \langle \, \cdot \, , \, \cdot \rangle^{1/2}.$ Let $\Gamma_0(\mathcal{H})$ be the set of proper lower semicontinuous convex functions from $\mathcal{H} \to (-\infty, \infty]$. Denote as $\mathbb{R}^{++}$ the (strictly) positive real line. Let $\mathcal{I}$ be the identity operator.
\begin{definition}[Fixed Points]
    Let $A: \mathcal{H} \to \mathcal{H}$ be an operator. The set of \textit{fixed points} for $A$ is
    \begin{equation}
        \text{Fix}\, A = \{ x \in \mathcal{H} \, : \, Ax = x\}.
    \end{equation}
\end{definition}

\begin{definition}[Argmin]
    Let $f : \mathcal{H} \to (-\infty, \infty]$ be proper and let $x \in \mathcal{H}$. Then $x$ is a \textit{minimizer} of $f$ if $f(x) = \inf f(\mathcal{H})$. The set of minimizers of $f$ is denoted $\text{Argmin} \, f$.
\end{definition}

\begin{definition}[Proximal Operators]
    Let $f: \mathcal{H} \to (-\infty, \infty]$ be a function. The \textit{proximal operator} associated with $f$ is given as
    \begin{equation}
        \text{Prox}_f(x) = \underset{u \in \mathcal{H}}{\text{Argmin}}\, f(u) + \frac{1}{2}\lVert u - x \rVert_2^2.
    \end{equation}
The proximal operator may be scaled with parameter $\gamma > 0$:
    \begin{equation}
        \text{Prox}_{\gamma f}(x) = \underset{u \in \mathcal{H}}{\text{Argmin}}\, f(u) + \frac{1}{2\gamma}\lVert u - x \rVert_2^2.
    \end{equation}
Importantly, if $f \in \Gamma_0(\mathcal{H})$, then $\text{Prox}_{\gamma f}$ is single-valued. 
\end{definition}

\begin{definition}[Subdifferential]
    Let $f \in \Gamma_0(\mathcal{H})$ and $x \in \mathcal{H}$. The \textit{subdifferential} of $f$ at $x$ is denoted by $\partial f(x)$ and is defined as:
    \begin{equation}
        \partial f(x) = \left\{g \in \mathcal{H} \, : \, \langle g, y - x \rangle + f(x) \leq f(y) \quad \forall y \in \mathcal{H}\right\}.
    \end{equation}
    The elements of the subdifferential $g$ are called \textit{subgradients}.
\end{definition}

\begin{definition}[Resolvent]
    Let $A: \mathcal{H} \to 2^{\mathcal{H}}$ be a set-valued operator and $\gamma \in \mathbb{R}^{++}$. The \textit{resolvent} of $A$ is 
    \begin{equation}
        J_{\gamma A} = (\mathcal{I} + \gamma A)^{-1},
    \end{equation}
    where $\mathcal{I}$ is the identity. The resolvent of the subdifferential of $f \in \Gamma_0(\mathcal{H})$ is the proximal operator of $f$:
    \begin{equation}
        J_{\gamma \partial f} = \text{Prox}_{\gamma f}.
    \end{equation}
\end{definition}

\begin{definition}[Reflected Resolvent]
    Let $A: \mathcal{H} \to 2^{\mathcal{H}}$ be a set-valued operator. The \textit{reflected resolvent} of $A$ is
    \begin{equation}
        R_{\gamma A} = 2J_{\gamma A} - \mathcal{I}.
    \end{equation}
\end{definition}

\begin{definition}[Nonexpansive]
    Let $D \subset \mathcal{H}$ and $T: D \to \mathcal{H}$. $T$ is \textit{nonexpansive} if
    \begin{equation}
        \lVert Tx - Ty \rVert \leq \lVert x - y \rVert \quad \forall x, y \in D.
    \end{equation}
\end{definition}

\begin{definition}[Firmly Nonexpansive]
    Let $D \subset \mathcal{H}$ and $T: D \to \mathcal{H}$. $T$ is \textit{firmly nonexpansive} if
    \begin{equation}
        \lVert Tx - Ty \rVert^2 + \lVert (\mathcal{I} - T)x - (\mathcal{I} - T)y \rVert^2 \leq \lVert x - y \rVert^2 \quad \forall x, y \in D.
    \end{equation}
\end{definition}

\section*{Lemmas}

\begin{lemma}
Let $f \in \Gamma_0(\mathcal{H})$ and $\gamma \in \mathbb{R}^{++}$. Then 
\begin{equation}
\text{Fix Prox}_f = \text{Fix Prox}_{\gamma f}.
\end{equation}
\end{lemma}
\begin{proof}
We have $\text{Argmin}\, f = \text{Argmin}\, \gamma f$. Since $f \in \Gamma_0(\mathcal{H})$, $\text{Argmin}\, f = \text{Fix Prox}_f$ (B\&C proposition 12.29). Hence
\begin{align*}
    \text{Fix Prox}_f = \text{Argmin}\, f &= \text{Argmin}\, \gamma f\\
    &=\text{Fix Prox}_{\gamma f}.
\end{align*}
\end{proof}
Note that this is why the proximal point algorithm isn't fussy about step sizes. The set of fixed points remains the same regardless, the step size simply changes convergence behavior.

\begin{lemma}\label{lemma:firm}
    Let $f \in \Gamma_0(\mathcal{H})$. $\text{Prox}_{\gamma f}$ is firmly nonexpansive for all $\gamma \in \mathbb{R}^{++}$. 
\end{lemma}

\begin{proof}
    Let $F = \partial f$. By B\&C theorem 20.25, $F$ is maximally monotone. Hence
    \[(\mathcal{I} + \gamma F)^{-1} = J_{\gamma F} = J_{\gamma \partial f} = \text{Prox}_{\gamma f}\]
    is firmly nonexpansive by B\&C proposition 23.8 ii.
\end{proof}

\begin{lemma}
    Let $f \in \Gamma_0(\mathcal{H})$. $R_{\gamma \partial f} = 2\text{Prox}_{\gamma f} - \mathcal{I}$ is nonexpansive for all $\gamma \in \mathbb{R}^{++}.$
\end{lemma}

\begin{proof}
    $\text{Prox}_{\gamma f}$ is firmly nonexpansive by Lemma \ref{lemma:firm}, apply B\&C proposition 4.4 iii).
\end{proof}

\begin{lemma}
    The composition of nonexpansive operators is nonexpansive.
\end{lemma}
\begin{proof}
Let $A, B$ be nonexpansive operators from $\mathcal{H} \to \mathcal{H}$, i.e. $\lVert Ax - Ay \rVert \leq \lVert x - y \rVert$ and $\lVert Bx - By \rVert \leq \lVert x - y \rVert \quad \forall x, y \in \mathcal{H}.$ Then
\begin{align*}
    \lVert ABx - ABy \rVert &\leq \lVert Bx - By \rVert \\
    &\leq \lVert x - y \rVert \quad \forall x, y \in \mathcal{H},
\end{align*}
so $AB$ is nonexpansive.
\end{proof}

\begin{lemma}
    $\text{Fix Prox}_{\gamma f} = \text{Fix}\, R_{\gamma\partial f}.$
\end{lemma}

\begin{proof}
    ($\Rightarrow$) Let $x \in \text{Fix Prox}_{\gamma f}.$ Then
    \begin{align*}
        R_{\gamma\partial f}x &= 2 \text{Prox}_{\gamma f}x - x \\
        &= 2x - x\\
        &= x,
    \end{align*}
    so $x \in \text{Fix}\, R_{\gamma\partial f}.$

    ($\Leftarrow$)  Let $x \in \text{Fix}\, R_{\gamma\partial f}.$ Hence
    \begin{align*}
        x &= R_{\gamma\partial f}x \\
        &= 2 \text{Prox}_{\gamma f}x - x \\
        2x &= 2 \text{Prox}_{\gamma f}x \\
        x &= \text{Prox}_{\gamma f}x,
    \end{align*}
    so $x \in \text{Fix Prox}_{\gamma f}.$ 
\end{proof}

\begin{lemma}[B\&C Lemma 2.17(ii).]
Let $(x, y) \in \mathcal{H} \times \mathcal{H}$.
\begin{align}
    \norm{x}^2 - \norm{2y - x}^2 &= 4 \left( \langle x, y \rangle - \norm{y}^2\right) \\
    &= 4 \langle x - y, y \rangle \\
    &= 2\left(\norm{x}^2 - \norm{x - y}^2 - \norm{y}^2\right).
    \label{bc217}
\end{align}
\end{lemma}

\begin{lemma}[B\&C Proposition 4.4]
    Let $D \subset \mathcal{H}$ and $T : D \to H$. The following are equivalent: 
    \begin{enumerate}
        \item $T$ is firmly nonexpansive.
        \item $\mathcal{I} - T$ is firmly nonexpansive.
        \item $2T - \mathcal{I}$ is nonexpansive.
        \item $\forall x, y \in D$, $\lVert Tx - Ty\rVert^2 \leq \langle x - y, Tx - Ty \rangle.$
        \item $\forall x, y \in D$, $0 \leq \langle Tx - Ty, \left(\mathcal{I} - T\right)x - \left(\mathcal{I} - T\right)y \rangle$. 
        \item $\forall x, y \in D$, $\forall \alpha \in [0,1],$ $\lVert Tx - Ty \rVert \leq \lVert\alpha(x - y) + (1 - \alpha)(Tx - Ty)\rVert.$
    \end{enumerate}
\end{lemma}

\begin{proof}
($1 \iff 2$). If $T$ is firmly nonexpansive, then 
\begin{equation*}
        \lVert Tx - Ty \rVert^2 + \lVert (\mathcal{I} - T)x - (\mathcal{I} - T)y \rVert^2 \leq \lVert x - y \rVert^2 \quad \forall x, y \in D.
\end{equation*}
Replace $T$ by $\mathcal{I} - T$, then the result is straightforward.

\vspace{1cm}
($1 \iff 3$). If $T$ is firmly nonexpansive then 
\begin{equation*}
        \lVert Tx - Ty \rVert^2 + \lVert (\mathcal{I} - T)x - (\mathcal{I} - T)y \rVert^2 \leq \lVert x - y \rVert^2 \quad \forall x, y \in D.
\end{equation*}
Rearrange this to
\begin{equation*}
        0 \leq \lVert x - y \rVert^2 - \lVert Tx - Ty \rVert^2 - \lVert (\mathcal{I} - T)x - (\mathcal{I} - T)y \rVert^2\quad \forall x, y \in D.
\end{equation*}
By \eqref{bc217} this is equivalent to
\begin{equation*}
    0 \leq \norm{x - y}^2 - \norm{2\left(Tx - Ty\right) - (x - y)}^2.
\end{equation*}
Consider the operator $S = 2T - \mathcal{I}$, this becomes
\begin{align*}
    0 &\leq \norm{x - y}^2 - \norm{Sx - Sy}^2 \\
    \norm{Sx - Sy}^2 &\leq \norm{x - y}^2.
\end{align*}
Taking the square root yields the condition for being nonexpansive. Hence $S = 2T-\mathcal{I}$ is nonexpansive. The reverse may be used from (3) to show (1).

\vspace{1cm}
($1 \iff 5$). If $T$ is firmly nonexpansive then 
\begin{equation*}
        \lVert Tx - Ty \rVert^2 + \lVert (\mathcal{I} - T)x - (\mathcal{I} - T)y \rVert^2 \leq \lVert x - y \rVert^2 \quad \forall x, y \in D.
\end{equation*}
Rearrange this to
\begin{equation*}
        0 \leq \lVert x - y \rVert^2 - \lVert Tx - Ty \rVert^2 - \lVert (\mathcal{I} - T)x - (\mathcal{I} - T)y \rVert^2\quad \forall x, y \in D.
\end{equation*}
By using \eqref{bc217} with $(x - y, Tx - Ty)$ this is equivalent to
\begin{equation*}
        0 \leq \langle Tx - Ty, (\mathcal{I} - T)x - (\mathcal{I} - T)y \rangle\quad \forall x, y \in D.
\end{equation*}
\end{proof}

\section*{AOI Line Search}
An averaged operator iteration has the form 
\begin{equation}
    x_{k+1} = x_k + \alpha\left(S x_k - x_k\right)
\label{eq:def_aoi}
\end{equation}
where $\alpha \in [0, 1]$ and $S$ is a non-expansive operator, i.e. $S$ satisfies $\norm{ Sx - Sy } \leq \norm{x - y}$. Gisselson et al.\ describe the following line search over the parameter $\alpha$ in an averaged operator iteration:
\begin{equation}
    \begin{aligned}
        r_k &= Sx_k - x_k \\
        \bar{x}_{k} &= x_k + \bar{\alpha} r_k \\
        \bar{r}_{k} &= S\bar{x}_k - \bar{x}_k \\
        x_{k+1} &= x_k + \alpha_kr_k.
    \end{aligned}
    \label{eq:aoi_linesearch_iters}
\end{equation}
Before running the algorithm, one sets a nominal step size $\bar{\alpha}$. In order, the steps of \eqref{eq:aoi_linesearch_iters} compute the current residual, compute the \textit{nominal} next step with the nominal step size, and then the residual with the nominal step size. The line search then occurs over the value of $\alpha_k$ in the final step. Either the step size is $\alpha_k = \bar{\alpha}$, the nominal step, or $\alpha_k \in (\bar{\alpha}, \alpha_{\text{max}}]$ is chosen such that
\begin{equation}
    \norm{r_{k+1}}_2 = \norm{Sx_{k+1} - x_{k+1}}_2 \leq (1 - \varepsilon)\norm{\bar{r}_{k}}_2,
    \label{eq:aoi_linesearch_cond}
\end{equation}
where $\varepsilon > 0$ and $\alpha_{\text{max}} > \bar{\alpha}$ are fixed algorithm parameters. 

We will be changing the step size in the operator $S$ as each step, so we will denote the operator as $S_k$. $S_k$ will be a composition of reflected resolvents, so the only thing changing at each step will be the parameter $\gamma$. $S_k$ will be nonexpansive for all steps $k$ by Lemma 3. The new iterations will be:

\begin{equation}
    x_{k+1} = x_k + \alpha\left(S_k x_k - x_k\right)
\label{eq:def_aoi}
\end{equation}
where $\alpha \in [0, 1]$. The following is a line search over the parameter $\alpha$ in an averaged operator iteration:
\begin{equation}
    \begin{aligned}
        r_k &= S_kx_k - x_k \\
        \bar{x}_{k} &= x_k + \bar{\alpha} r_k \\
        \bar{r}_{k} &= S_k\bar{x}_k - \bar{x}_k \\
        x_{k+1} &= x_k + \alpha_kr_k.
    \end{aligned}
    \label{eq:aoi_linesearch_iters}
\end{equation}

For this to be PDHG with line search, $S_k = R_{(\gamma \partial g)^{-1}}R_{\gamma \partial f},$ a composition of reflected resolvents. 
\section*{Theorems}
\begin{theorem}
    Let $S_k: \mathcal{H} \to \mathcal{H}$ be nonexpansive. Then the iterations \eqref{eq:aoi_linesearch_iters} satisfy $\norm{r_{k}}_2 \to c$ as $k \to \infty.$
\end{theorem}

\begin{proof}
There are two cases to check: $\alpha_k = \bar{\alpha}$ and $\alpha_k > \bar{\alpha}.$
    First, consider $\alpha_k = \bar{\alpha}$. Denote $T_k = (1 - \bar{\alpha})\mathcal{I} - \bar{\alpha}S_k.$ The update for $\bar{x}_k$ is then
    \begin{align*}
        \bar{x}_k = x_k + \bar{\alpha}r_k &= x_k + \bar{\alpha}\left(S_kx_k - x_k\right)\\
        &= (1 - \bar{\alpha})x_k + \bar{\alpha}S_kx_k \\
        &= T_kx_k.
    \end{align*}
    Since $\alpha_k = \bar{\alpha}$, $x_{k+1} = \bar{x}_k$, 
    \[\norm{r_{k+1}} = \norm{\bar{r}_k}.\]
    This gives us
    \begin{align*}
        \norm{r_{k+1}} = \norm{\bar{r}_k} &= \norm{\bar{x}_k - S_k\bar{x}_k } \\
        &= \frac{1}{\bar{\alpha}} \norm{\bar{x}_k - T_k\bar{x}_k} \\
        &= \frac{1}{\bar{\alpha}}\norm{T_kx_k - T_kT_kx_k},
    \end{align*}
    since $\norm{x - T_kx} = \norm{x - (1 - \bar{\alpha})x - \bar{\alpha}S_kx} = \bar\alpha\norm{x - S_kx}.$
    Since $T_k$ is nonexpansive for all $k$ (by Lemmas 3 \& 4), we have
    \begin{align*}
        \norm{r_{k+1}} &= \frac{1}{\bar{\alpha}}\norm{T_kx_k - T_kT_kx_k} \\
        &\leq \frac{1}{\bar{\alpha}}\norm{x_k - T_kx_k} \\
        &= \norm{x_k - S_kx_k} = \norm{r_k}.
    \end{align*}

    Now assume $\alpha_k > \bar{\alpha}$. Then by the line search condition \eqref{eq:aoi_linesearch_cond}
    \begin{equation}
        \norm{r_{k+1}} \leq (1 - \varepsilon)\norm{\bar{r}_k} \leq (1 - \varepsilon)\norm{r_k}.
    \end{equation}
    So $\{r_k\}_{k=1}^{\infty}$ are a decreasing sequence and bounded below by $0$ and so it converges.
\end{proof}

\newpage
\section*{Pairwise Nonexpansive Operators}
\subsection*{Definitions}
\begin{definition}[Pairwise Nonexpansive Operators]
Let $T_1, T_2: \mathcal{H} \to \mathcal{H}$. They are \textit{pairwise nonexpansive} if
\begin{equation}
    \lVert T_1 x - T_2 y \rVert \leq \lVert x - y \rVert \quad \forall x, y \in \mathcal{H}.
\end{equation}
\end{definition}

\begin{definition}[Pairwise Firmly Nonexpansive Operators]
Let $T_1, T_2: \mathcal{H} \to \mathcal{H}$. They are \textit{pairwise firmly nonexpansive} if
\begin{equation}
    \lVert T_1 x - T_2 y \rVert^2 + \lVert \left(\mathcal{I} - T_1\right)x - \left(\mathcal{I} - T_2\right)y \rVert^2 \leq \lVert x - y \rVert^2 \quad \forall x, y \in \mathcal{H}.
\end{equation}
\end{definition}

\subsection*{Lemmas}
\begin{lemma}[B\&C Lemma 2.17 (ii) for Multiple Operators]
Apply \eqref{bc217} with $(x - y, T_1x - T_2y)$:
\begin{align}
    \norm{x - y}^2 &- \norm{2(T_1x - T_2y) - (x - y)}^2 \\
    &= 4\left(\langle x - y, T_1x - T_2y \rangle - \norm{T_1x - T_2y}^2 \right) \\
    &= 4 \langle x - y - (T_1x - T_2y), T_1x - T_2y \rangle \\
    &= 2\left(\norm{x - y}^2 - \norm{x - y - (T_1x - T_2y)}^2 - \norm{T_1x - T_2y}^2\right).
    \label{eq:bc217_mult}
\end{align}
\end{lemma}

\begin{lemma}[B\&C Proposition 4.4 for Pairwise Nonexpansive Operators]\label{lemma:4.4_pairwise}
    Let $D \subset \mathcal{H}$ and $T_1, T_2 : D \to H$. The following are equivalent: 
    \begin{enumerate}
        \item $T_1, T_2$ are pairwise firmly nonexpansive.
        \item $\mathcal{I} - T_1$ and $\mathcal{I} - T_2$ are pairwise firmly nonexpansive.
        \item $2T_1 - \mathcal{I}$ and $2T_2 - \mathcal{I}$ are pairwise nonexpansive.
        \item $\forall x, y \in D$, $\lVert T_1x - T_2y\rVert^2 \leq \langle x - y, T_1x - T_2y \rangle.$
        \item $\forall x, y \in D$, $0 \leq \langle T_1x - T_2y, \left(\mathcal{I} - T_1\right)x - \left(\mathcal{I} - T_2\right)y \rangle$. 
        \item $\forall x, y \in D$, $\forall \alpha \in [0,1],$ $\lVert T_1x - T_2y \rVert \leq \lVert\alpha(x - y) + (1 - \alpha)(T_1x - T_2y)\rVert.$
    \end{enumerate}
\end{lemma}

\begin{proof}
$(1 \iff 2)$. $T_1, T_2$ being pairwise firmly nonexpansive means that
    \begin{equation}
    \lVert T_1 x - T_2 y \rVert^2 + \lVert \left(\mathcal{I} - T_1\right)x - \left(\mathcal{I} - T_2\right)y \rVert^2 \leq \lVert x - y \rVert^2 \quad \forall x, y \in \mathcal{H}.
\end{equation}
Replace $T_1, T_2$ by $\mathcal{I} - T_1$ and $\mathcal{I} - T_2$ and the result still holds, hence $\mathcal{I} - T_1$ and $\mathcal{I} - T_2$ are pairwise firmly nonexpansive.

\vspace{1cm}
\noindent
    $(1 \iff 3)$. $T_1, T_2$ being pairwise firmly nonexpansive means that
    \begin{equation}
    \lVert T_1 x - T_2 y \rVert^2 + \lVert \left(\mathcal{I} - T_1\right)x - \left(\mathcal{I} - T_2\right)y \rVert^2 \leq \lVert x - y \rVert^2 \quad \forall x, y \in \mathcal{H}.
\end{equation}
Rearrange to
\begin{equation}
    0 \leq \lVert x - y \rVert^2 - \lVert T_1 x - T_2 y \rVert^2 - \lVert \left(\mathcal{I} - T_1\right)x - \left(\mathcal{I} - T_2\right)y \rVert^2  \quad \forall x, y \in \mathcal{H}.
\end{equation}
By \eqref{eq:bc217_mult} this is equivalent to
\begin{equation}
    0 \leq \norm{x - y}^2 - \norm{2(T_1x - T_2y) - (x - y)}^2  \quad \forall x, y \in \mathcal{H},
\end{equation}
or equivalently 
\begin{equation}
    \norm{2(T_1x - T_2y) - (x - y)}^2 \leq \norm{x - y}^2   \quad \forall x, y \in \mathcal{H},
\end{equation}
which is the condition for $2T_1 - \mathcal{I}$ and $2T_2 - \mathcal{I}$ to be pairwise nonexpansive. 

\vspace{1cm}
\noindent
$(1 \iff 5)$. $T_1, T_2$ being pairwise firmly nonexpansive means that
    \begin{equation}
    \lVert T_1 x - T_2 y \rVert^2 + \lVert \left(\mathcal{I} - T_1\right)x - \left(\mathcal{I} - T_2\right)y \rVert^2 \leq \lVert x - y \rVert^2 \quad \forall x, y \in \mathcal{H}.
\end{equation}
By \eqref{eq:bc217_mult} this is equivalent to
\begin{equation}
    0 \leq \langle x - y - (T_1x - T_2y), T_1x - T_2y \rangle \quad \forall x, y \in \mathcal{H}.
\end{equation}
\end{proof}

\begin{lemma}
    The composition of pairwise nonexpansive operators is pairwise nonexpansive.
    Let $\left\{T_i\right\}_{i=1}^{\infty}$ be a family of pairwise nonexpansive operators on $\mathcal{H}$. Then the composition of any two, i.e. $T_i \circ T_j$, is also pairwise nonexpansive.
\end{lemma}
\begin{proof}
    Let $T_i, T_j, T_k, T_l$ be pairwise nonexpansive operators and let $x, y \in \mathcal{H}$. Without loss of generality, 
    \begin{align*}
        \norm{T_iT_jx - T_kT_ly} \leq \norm{T_jx - T_ly} \leq \norm{x - y},
    \end{align*}
    so arbitrary compositions of pairwise nonexpansive operators remain pairwise nonexpansive.
\end{proof}
\begin{lemma}[B\&C Proposition 12.26]
    Let $f \in \Gamma_0(\mathcal{H})$ and $x, p \in \mathcal{H}$. Then
    \begin{equation}
        p = \text{Prox}_{f}x \iff (\forall y \in \mathcal{H}) \quad \langle y - p, x - p \rangle + f(p) \leq f(y).
    \end{equation}
    \label{bc_1226}
\end{lemma}

\subsection*{Theorems}
\begin{theorem}
    Let $f \in \Gamma_0(\mathcal{H})$ and $\gamma, \mu \in \mathbb{R}^{++}.$ Then $\text{Prox}_{\gamma f}$ and $\text{Prox}_{\mu f}$ are pairwise firmly nonexpansive.
\end{theorem}
\begin{proof}
    Let $x, y \in \mathcal{H}$ and $\gamma, \mu \in \mathbb{R}^{++}$. Denote
    \begin{align*}
        p &= \text{Prox}_{\gamma f}x \\
        q &= \text{Prox}_{\mu f}y.
    \end{align*}
    By B\&C Proposition 12.26 (Lemma \ref{bc_1226}) we have
    \begin{align*}
        \langle q - p, x - p \rangle + f(p) &\leq f(q) \\
        \langle p - q, y - q \rangle + f(q) &\leq f(p).
    \end{align*}
    Summing these inequalities yields
    \begin{align*}
        0 &\leq -\langle q - p, x - p \rangle - \langle p - q, y - q \rangle \\
        &= \langle p - q, (x - p) - (y - q) \rangle \\
        &= \langle \text{Prox}_{\gamma f}x  - \text{Prox}_{\mu f}y, \left(\mathcal{I} - \text{Prox}_{\gamma f}\right) x - \left(\mathcal{I} - \text{Prox}_{\mu f}\right)y \rangle.
    \end{align*}
    This holds for all $x, y \in \mathcal{H}$ so by Lemma \ref{lemma:4.4_pairwise}, 
    $\text{Prox}_{\gamma f}$ and $\text{Prox}_{\mu f}$ are pairwise firmly nonexpansive for all $\gamma, \mu \in \mathbb{R}^{++}$.
\end{proof}

\begin{theorem}
    The operator $S = R_{(\gamma G)^{-1}}R_{\gamma F}$ for PDHG with line search is pairwise nonexpansive for all $\gamma \in \mathbb{R}^{++}$.
\end{theorem}
\begin{proof}
    For functions $f, g \in \Gamma_0(\mathcal{H})$, let $F = \partial f$ and $G = \partial g$. The operator $S$ is
    \begin{align*}
        S = R_{(\gamma G)^{-1}}R_{\gamma F} = R_{(\gamma\partial g)^{-1}}R_{\gamma\partial f}.
    \end{align*}
    The operator $R_{\gamma\partial f} = 2J_{\gamma\partial f} - \mathcal{I}$ is the \textit{reflected resolvent} of the subdifferential. The resolvent $J_{\gamma\partial f}$ is the prox operator of $f$, and so it is firmly nonexpansive. Furthermore, it is pairwise firmly nonexpansive with all other $J_{\mu\partial f}$ for $\mu \in \mathbb{R}^{++}$ by Theorem 2. Hence the reflected resolvent $R_{\gamma\partial f}$ is pairwise nonexpansive for all $\gamma \in \mathbb{R}^{++}$ by Lemma 9. 

    By Lemma 10, the composition of pairwise nonexpansive operators is pairwise nonexpansive, so $S_{\gamma} = R_{(\gamma\partial g)^{-1}}R_{\gamma\partial f}$ is pairwise nonexpansive for all $\gamma \in \mathbb{R}^{++}$. By Theorem 4, the iteration
    \[x_{n+1} = x_n + \lambda_n(S_nx_n - x_n)\]
    converges.
\end{proof}

\begin{theorem} [B\&C Thm 5.15]
    Let $\{T_n\}_{n=1}^{\infty}$ be a family of operators such that $T_i$ and $T_j$ are pairwise nonexpansive for all $i, j \in \mathbb{N}$. Let $\text{Fix}\,T = \bigcap_{i}\text{Fix}\,T_i$ be the intersection of the sets of fixed points and assume $\text{Fix}\,T \neq \varnothing$. Let $\{\lambda_n\}_{n \in \mathbb{N}}$ be a sequence in $[0, 1]$ such that $\sum_{n\in\mathbb{N}}\lambda_n(1-\lambda_n) = +\infty$. Let our iteration be
    \begin{equation}
        x_{n+1} = x_n + \lambda_n\left(T_nx_n - x_n\right).
        \label{eq:proof_iter}
    \end{equation}
    Then:
    \begin{enumerate}
        \item $\{x_n\}_{n \in \mathbb{N}}$ is Fejer monotonic to $\text{Fix} \, T$. 
        \item $\left(T_nx_n - x_n\right)_{n \in \mathbb{N}}$ converges strongly to $0$.
        \item $\{x_n\}_{n\in\mathbb{N}}$ converges weakly to a point in $\text{Fix} \, T.$
    \end{enumerate}
\end{theorem}

\begin{proof}

(1).
    Let $y \in \text{Fix}\, T$. Then
    \begin{align*}
        \norm{x_{n+1} - y}^2 &= \norm{(1 - \lambda_n)x_n + \lambda_nT_nx_n - y}^2 \\
        &= \norm{(1 - \lambda_n)(x_n - y) + \lambda_nT_nx_n - \lambda_ny}^2 \\
        &= \norm{(1 - \lambda_n)(x_n - y) + \lambda_nT_n(x_n - y)}^2 \\
        &= (1 - \lambda_n)\norm{x_n - y}^2 + \lambda_n \norm{T_nx_n - T_ny}^2 \\
        &- \lambda_n(1 - \lambda_n)\norm{T_nx_n - x_n}^2 \\
        &\leq \norm{x_n - y}^2 - \lambda_n(1-\lambda_n)\norm{T_nx_n - x_n}^2.
    \end{align*}
    Hence $\{x_n\}$ is Frejer monotone to $\text{Fix}\, T$. Further, 
    \[\sum_{n \in \mathbb{N}}\lambda_n(1-\lambda_n)\norm{T_nx_n - x_n}^2 \leq \norm{x_0 - y}^2.\]
    Since $\sum_{n\in\mathbb{N}}\lambda_n(1-\lambda_n) = +\infty$, hence $\lim_{n\to \infty}\norm{T_nx_n - x_n} \to 0$.

(2).
The iterations \eqref{eq:proof_iter} may also be written
\begin{equation}
    x_{n+1} = (1 - \lambda_n)x_n + \lambda_nT_nx_n.
\end{equation}

\begin{align*}
    \norm{T_{n+1}x_{n+1} - x_{n+1}} &= \norm{T_{n+1}x_{n+1} - \left[(1 - \lambda_n)x_n + \lambda_nT_nx_n\right]} \\
    &= \norm{T_{n+1}x_{n+1} - T_nx_n + T_nx_n - \lambda_nT_nx_n - (1-\lambda_n)x_n} \\
    &= \norm{T_{n+1}x_{n+1} - T_nx_n + (1-\lambda_n)T_nx_n - (1- \lambda_n)x_n} \\
    &\leq \norm{T_{n+1}x_{n+1} - T_nx_n} + (1-\lambda_n)\norm{T_nx_n - x_n} \\
    &\leq \norm{x_{n+1} - x_n} + (1 - \lambda_n)\norm{T_nx_n - x_n} \\
    &= \lambda \norm{T_nx_n - x_n} + (1 - \lambda_n)\norm{T_nx_n - x_n} \\
    &= \norm{T_nx_n - x_n}.
\end{align*}
Thus $\norm{T_nx_n - x_n}$ converges. Since $\lim_{n \to \infty} \norm{T_nx_n - x_n} \to 0$ hence $\{T_nx_n - x_n\}_{n \in \mathbb{N}} \to 0.$ 

(3). 
By Corollary 4.28 in B\&C, $\{x_n\}_{n\in\mathbb{N}}$ converges weakly to a point in $\text{Fix} \, T.$
\end{proof}
Hence the iterations converge and so the residuals from Theorem 1 converge to 0.


==> app3_pddrpdhg.tex <==
\newpage
\section{The Connection Between PDDR and PDHG}\label{ap:3}
This result is shown in \cite{o2020equivalence} which we include here for completeness.

\subsection{PDHG Iterations}
The PDHG iterations follow:
\begin{equation}
\begin{aligned}
\bar{x}_k &= J_{\tau F}\left(x_{k-1} - \tau A^{*}z_{k-1}\right) \\
\bar{z}_k &= J_{\sigma G^{-1}}\left(z_{k-1} + \sigma A(2\bar{x}_k - x_{k-1]})\right) \\
x_k &= (1 - \rho_k)x_{k-1} + \rho_k\bar{x}_k\\
z_k &= (1 - \rho_k)z_{k-1} + \rho_k\bar{z}_k.
\end{aligned}
\label{app:pdhg_iters}
\end{equation}

The iterations from Douglas Rachford follow:
\begin{equation}
\begin{aligned}
x_{k+1} &= J_{\gamma F}(y_k) \\
w_{k+1} &= J_{\gamma G}(2x_{k+1} - y_k)\\
y_{k+1} &= y_k + \rho_k(w_{k+1} - x_{k+1}).
\end{aligned}
\label{app:dr}
\end{equation}

Using the relationship between resolvents in step 2 yields the \textit{primal dual} formulation of Douglas Rachford:
\begin{equation}
\begin{aligned}
    x_{k+1} &= J_{\gamma F}(y_k) \\
    w_{k+1} &= J_{(\gamma G)^{-1}}(2x_{k+1} - y_k) \\
    y_{k+1} &= (1 - \rho_k)y_k + \rho_k(x_{k+1} - w_{k+1}).
\end{aligned}
\label{app:pddr}
\end{equation}

\subsection{The Modified Problem}
The original problem we want to solve is
\begin{equation}
\underset{x\in\mathcal{H}^1}{\text{minimize}} \, f(x) + g(Ax),
\label{app:primal}
\end{equation}
where $A: \mathcal{H}^1 \to \mathcal{H}^2$, and $\mathcal{H}^1, \mathcal{H}^2$ may be separate Hilbert spaces. For the remainder of this section we will have partitioned variables, e.g. $x = (x_1, x_2)$ where $x_1 \in \mathcal{H}^1$ and $x_2 \in \mathcal{H}^2$. 

We define the \textit{modified problem} as
\begin{equation}
\underset{\tilde{x}\in\mathcal{H}}{\text{minimize}} \, \tilde{f}(x) + \tilde{g}(x)
\label{app:modified}
\end{equation}
where $\tilde{f}$ and $\tilde{g}$ are defined:
\begin{equation}
\tilde{f}(x_1, x_2) = \begin{cases} f(x_1) \quad &\text{if }x_2 = 0 \\ \infty \quad &\text{otherwise} \end{cases}, \qquad \tilde{g}(x_1, x_2) = g(Ax_1 + Bx_2),
\label{def:tildefunctions}
\end{equation}
where now $B$ is chosen such that $AA^* + BB^* = \frac{1}{\theta}\mathcal{I}$. 

Let $\tilde{x} = [x_1 \;x_2]^*$ and $C = [A \;B]$, this becomes

\begin{equation}
\text{minimize}\, \tilde{f}(\tilde{x}) + g(C\tilde{x}),
\end{equation}
where $CC^* = AA^* + BB^* = \frac{1}{\theta}\mathcal{I}$ and
\begin{equation}
\tilde{f}(\tilde{x}) = f(x_1) + \delta_{\{0\}}(x_2).
\label{app:f_tilde}
\end{equation}
Hence this second term now has a proximal operator in closed form given by \eqref{def:prox_composed}. Therefore we can apply PDDR to this problem since we can now evaluate both $J_{\gamma F}$ and $J_{\left(\gamma G\right)^{-1}}$.

The second term of $\tilde{f}$ ensures that $x_2 = 0$ for all iterations of whatever iterative algorithm we use to solve the problem. The proximal operator of $\tilde{f}$ then is separable and we can write (with $y = (y_1, y_2)$)
\begin{equation}
\prox_{\gamma\tilde{f}}(y) = \left(\prox_{\gamma f}(y_1), 0\right).
\label{app:proxftilde}
\end{equation}

The expression for the proximal operator of $\tilde{g}$ comes from \eqref{def:prox_composed}:
\begin{equation}
J_{\gamma\tilde{G}}(y) = \prox_{\gamma \tilde{g}}(y) = \, y + \alpha C^*\left(\prox_{\sigma^{-1} g}(Cy) - Cy\right),
\label{app:proxgtilde}
\end{equation}
where $\sigma = \alpha / \gamma$. From the definition of scalar multiplication and inverse of monotone operators, we get the resolvent of $(\tau \tilde{G})^{-1}$ as
\begin{equation}
J_{(\tau\tilde{G}^{-1})}(y) = \tau C^*J_{\sigma G^{-1}}(\sigma C y).
\label{app:proxgtildeconj}
\end{equation}

\subsection{To PDHG}

The new variables for the modified problem are in a hybrid space (assumed $n + p$ dimensional) which we will partition into $x_k = (x_{k_1}, x_{k_2})$, $w_k = (w_{k_1}, w_{k_2})$, and $y_k = (y_{k_1}, y_{k_2})$.

The iterations for PDDR applied to the modified problem yield:
\begin{equation}
\begin{aligned}
x_{k+1} &= J_{\tau \tilde{F}}(y_k) \\
w_{k+1} &= J_{(\tau\tilde{G})^{-1}} (2x_{k+1} - y_{k}) \\
y_{k+1} &= (1 - \rho_k)y_k + \rho_k(x_{k+1} - w_{k+1}).
\end{aligned}
\end{equation}

Using the expressions for the two resolvents \eqref{app:proxftilde} and \eqref{app:proxgtilde} we get
\begin{equation}
\begin{aligned}
x_{k+1} &= \left(J_{\gamma F}(y_{k_1}), 0\right) \\
w_{k+1} &= \tau C^*J_{\sigma G^{-1}}(\sigma C(2x_{k+1} - y_{k}) \\
y_{k+1} &= (1 - \rho_k)y_{k} + \rho_k(w_{k+1} - x_{k+1}),
\end{aligned}
\label{app:pddr2}
\end{equation}
where as before $\sigma = \alpha / \tau$. 

Now we introduce two new variables, $u_k = (1 - \rho_k)u_{k-1} + \rho_kx_k$ and $z_k = u_k - y_k$, we get

\begin{align}
x_{k+1} &= \left(J_{\gamma F}(y_{k_1}), 0\right) \\
w_{k+1} &= \tau C^*J_{\sigma G^{-1}}(\sigma C(2x_{k+1} - y_{k}) \\
u_{k+1} &= (1 - \rho_k)u_{k-1} + \rho_ku_k \label{app:eq3}\\
y_k &= (1 - \rho_k)y_{k-1} + \rho_k(x_k - w_k) \label{app:eq4}\\
z_k &= u_k - y_k 
\label{app:pddr3}
\end{align}

The variable $y_k$ can now be eliminated. If we subtract \eqref{app:eq4} from \eqref{app:eq3} then the $w$ update in \eqref{app:eq3} becomes
\begin{equation}
w_k = (1 - \rho_k)(u_{k-1} - y_{k-1}) + \rho_k\bar{w}_k = (1 - \rho_k)w_{k-1} + \rho_k\bar{w}_k.
\end{equation}
Then, substituting $y_{k-1} = u_{k-1} - w_{k-1}$ in the first and second steps of the algorithm and removing the update in \eqref{app:eq4}:

\begin{equation}
\begin{aligned}
\bar{u}_k &= \left(J_{\gamma F}(u_{{k-1}_1}  - w_{{k-1}_1}),0\right)\\
\bar{w}_k &= \tau C^{*}J_{\sigma G^{-1}}\left(\sigma Cw_{k-1} + \sigma C(2\bar{u}_{k} - u_{k-1})\right) \\
u_k &= (1 - \rho_k)u_{k-1} + \rho_k \bar{u}_k \\
w_k &= (1 - \rho_k) w_{k-1} + \rho_k\bar{w}_k.
\end{aligned}
\end{equation}
The expression on the first line shows that $\bar{u}_{k_2} = 0$ for all $k$. If we start with our first iteration $u_{0_2}$ then line 3 shows that also $u_{k_2} = 0$ for all $k$. The expression on the second line shows that $\bar{w}_k$ is in the range of $C^{*}$ for all $k$; i.e. $\bar{w}_k = \tau C^{*}\bar{z}_k$ for some $\bar{z}_k$. If we choose $w_0$ in the range of $C^{*}$ then the final line shows that $w_k$ is also in the range of $C^{*}$ for all $k$, i.e. $w_k = \tau C^{*} z_k$ for some $z_k$. Since $CC^{*} = \alpha^{-1}\mathcal{I}$, the vectors $\bar{z}_k$ and $z_k$ are uniquely defined and equal to
\begin{align*}
\bar{z}_k &= (\alpha / \tau)C\bar{w}_k = \sigma C\bar{w}_k, \\
z_k &= (\alpha / \tau)Cw_k = \sigma Cw_k.
\end{align*}
Making these substitutions we can write the iterations as

\begin{equation}
\begin{aligned}
\bar{x}_k &= J_{\tau F}\left(x_{k-1} - \tau A^{*}z_{k-1}\right) \\
\bar{z}_k &= J_{\sigma G^{-1}}\left(z_{k-1} + \sigma A(2\bar{x}_k - x_{k-1})\right) \\
x_k &= (1 - \rho_k)x_{k-1} + \rho_k\bar{x}_k \\
z_k &= (1 - \rho_k)z_{k-1} + \rho_k\bar{z}_k.
\end{aligned}
\label{app:pdhg}
\end{equation}





==> app4_ops.tex <==
\section{Monotone Operator Relationships}
For the remainder of this section, let $F, G$ be monotone operators on a Hilbert space $\mathcal{H}$. 

\subsection{Graph}
The \textit{graph} of an operator is defined as\todo{check if you already }
\begin{equation}
\text{gr{A}} = \left\{(x, y) \, \vert \, y \in A(x)\right\}
\end{equation}

The relationship between the graph of $A$ and its inverse is then
\begin{equation}
\text{gr}(A^{-1}) = \begin{bmatrix} 0 & \mathcal{I} \\ \mathcal{I} & 0 \end{bmatrix} \text{gr}(A).
\end{equation}

{\large \textbf{resolvents, reflected resolvents, scalar mult}}
